Resilient Self-Debugging Software Protection

Debuggers are a popular reverse engineering and tampering tool. Self-debugging is an effective technique for applications to defend themselves against hostile debuggers. In penetration tests on state-of-the-art self-debugging, we observed several opportunities through which it could be attacked, however. We therefore improved upon the existing technique, making it more resilient by introducing reciprocal debugging and making the transfers of control between protected application and self-debugger more stealthy. This paper presents the improved self-debugging design, and details our research efforts into realizing reciprocal debugging. In our evaluation we show that the improved design is significantly harder for attackers to defeat.

==> related.tex <==
\section{Related Work}

Many anti-debugging techniques exist. Most of them consist of consist of dynamic checks to query the run-time environment for signs of active debugging, and are
easy to counter~\cite{FerrisAntiDebugging2011,beginnersantidebugging,collbergsurreptitious}. Self-debugging is a stronger, more complex anti-debugging technique
where the single available debugger seat for the protected application is occupied by a friendly debugger that cannot trivially be replaced by a hostile
debugger~\cite{StarCraft2,nanomites}. The technique which this paper builds on was a much improved, tightly coupled version of
self-debugging~\cite{abrath2016tightly}.

Related to our technique, the \verb!PTRACE_O_EXITKILL! option we employ in our design has another use case: jailers~\cite{ptrace}. Using this option ensures
that a debugged process can never escape its debugger's control, even if the debugger unexpectedly exits.

% talk about popov2007binary
% code reuse, factoring, for application code being executed also in context of switch to mini-debugger?
% data obfuscation?

% vim: set textwidth=160:

